ResponsibleRobotBench: Benchmarking Risk-Aware Task-Level Decision Making for Robotic Manipulation with Large Multimodal Models

Safe task-level manipulation requires a planner to recognize hazards, select appropriate mitigation actions, and satisfy their execution prerequisites without abandoning the original goal. We introduce ResponsibleRobotBench, a benchmark of 23 manipulation task configurations with separately specified goals and safety conditions. It connects hazard-category predictions, planned actions, execution feedback, and terminal outcomes at the episode level. Across evaluations of five large multimodal models, terminal safety and safe task completion can diverge: defense prompts increase terminal safety for three tested models but affect safe success in different directions. Correct hazard-category predictions also fail to ensure executable mitigation. In a cutting task under the default configuration, GPT-4o mini identifies the human hazard in all 100 episodes but never requests assistance, and every episode ends unsafe. Offering a help action and actually requesting it lead to different comparisons: outcomes differ between action menus even for a model that never requests help, and repeated requests can leave execution failures unresolved. Imitation-learning evaluations and physical robot sequences illustrate the need to coordinate mitigation with goal actions. Together, these results motivate evaluating mitigation selection, action prerequisites, and recovery alongside hazard recognition and terminal outcomes. The appendix provides task definitions, checker conditions, and prompts. Project website: https://responsible-robot-benchmark.github.io/.

==> tab/table_style.tex <==
% Restrained color hierarchy shared by both manuscript languages and appendix.
\RequirePackage{colortbl}
\definecolor{RRBHeader}{HTML}{E7EDF5}
\definecolor{RRBStripe}{HTML}{F5F7FA}
\definecolor{RRBAccent}{HTML}{F0EAF6}
\definecolor{RRBPositive}{HTML}{628C66}
\definecolor{RRBMuted}{RGB}{111,121,133}
\DeclareRobustCommand{\RRBYes}{\textcolor{RRBPositive}{\ensuremath{\checkmark}}}
\DeclareRobustCommand{\RRBNo}{\textcolor{RRBMuted}{\ensuremath{\square}}}

\DeclareRobustCommand{\RRBWorkingMark}[1]{%
  \ifdefined\RRBCleanCopy #1\else\textcolor{red}{#1}\fi}
\providecommand{\RRBWorkingRate}[2]{\RRBWorkingMark{#2}}

